A Survey on Asking Clarification Questions Datasets in Conversational Systems

The ability to understand a user's underlying needs is critical for conversational systems, especially with limited input from users in a conversation. Thus, in such a domain, Asking Clarification Questions (ACQs) to reveal users' true intent from their queries or utterances arise as an essential task. However, it is noticeable that a key limitation of the existing ACQs studies is their incomparability, from inconsistent use of data, distinct experimental setups and evaluation strategies. Therefore, in this paper, to assist the development of ACQs techniques, we comprehensively analyse the current ACQs research status, which offers a detailed comparison of publicly available datasets, and discusses the applied evaluation metrics, joined with benchmarks for multiple ACQs-related tasks. In particular, given a thorough analysis of the ACQs task, we discuss a number of corresponding research directions for the investigation of ACQs as well as the development of conversational systems.

==> sections/07-conclusion.tex <==
\section{Conclusion}
%Asking Clarification Questions has attracted increasing research attention. 
In this paper, we have presented the most recent and largest review of publicly available datasets used in ACQs. We first introduced a formal definition of ACQs, then provided background information about the way each dataset was created and the tasks that they define. This survey summarizes current research efforts and trends and we expect it can facilitate future research in the community.
